An Introduction to Simulation-Based Techniques for Automated Service Composition

This work is an introduction to the author's contributions to the SOC area, resulting from his PhD research activity. It focuses on the problem of automatically composing a desired service, given a set of available ones and a target specification. As for description, services are represented as finite-state transition systems, so to provide an abstract account of their behavior, seen as the set of possible conversations with external clients. In addition, the presence of a finite shared memory is considered, that services can interact with and which provides a basic form of communication. Rather than describing technical details, we offer an informal overview of the whole work, and refer the reader to the original papers, referenced throughout this work, for all details.

==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{37}
\providecommand{\eid}{4}

